Trajectory-aligned Space-time Tokens for Few-shot Action Recognition

We propose a simple yet effective approach for few-shot action recognition, emphasizing the disentanglement of motion and appearance representations. By harnessing recent progress in tracking, specifically point trajectories and self-supervised representation learning, we build trajectory-aligned tokens (TATs) that capture motion and appearance information. This approach significantly reduces the data requirements while retaining essential information. To process these representations, we use a Masked Space-time Transformer that effectively learns to aggregate information to facilitate few-shot action recognition. We demonstrate state-of-the-art results on few-shot action recognition across multiple datasets. Our project page is available at https://www.cs.umd.edu/~pulkit/tats

==> sections/old_2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\pk{remove d2st}

\subsubsection{Few-shot action recognition.}

In comparison to few-shot image classification, few-shot action recognition is a considerably more intricate task since it deals with higher-dimension video data characterized by enriched spatio-temporal context interactions and temporal variations \cite{kliper2011one, poppe2010survey, wang2021proposal, wang2021self}. The prevalent approach among existing few-shot action recognition methods is to apply the metric-based learning paradigm, but with different focuses.
% which aims to temporally match frames for simple yet effective classification. 
Some methods focus on feature representation enhancement and spatio-temporal modeling \cite{strm, sloshnet, hyrsm, mtfan, zhu2018compound, zhu2020label}. For instance, CMN \cite{zhu2018compound} integrates a memory structure and multi-saliency algorithm to encode video representations and models the temporal features through hand-designed temporal alignment algorithms. MTFAN \cite{mtfan} and HyRSM \cite{hyrsm} prioritize task-specific feature learning with MTFAN using a motion encoder to integrate global motion patterns while HyRSM uses hybrid relation modeling. GgHM \cite{gghm} also learns task-oriented features by optimizing intra- and inter-class feature correlations explicitly. SloshNet \cite{sloshnet} employs a feature fusion module automatically combines low-level and high-level spatial features, while a long-term temporal modeling module captures global temporal relations from spatial appearance features. Other methods focus on class prototype matching strategies / \textcolor{red}{designing effective metric learning strategies} \cite{otam, trx, hyrsm, hyrsm++, hcl, bishay2019tarn, zhang2021learning, zhang2020few, wang2021semantic, ni2022multimodal, d2st, fu2020depth, ni2022multimodal}. OTAM \cite{otam} uses a differentiable dynamic time warping algorithm \cite{muller2007dynamic} with an ordered temporal alignment for estimating distance between the query video and the support set videos. ARN \cite{zhang2020few} introduces a self-supervised permutation invariant strategy and learns long-range temporal dependencies by building on a 3D backbone \cite{tran2015learning}. TRX \cite{trx} matches each query sub-sequence with all sub-sequences in the support set to classify actions. ITANET \cite{zhang2021learning} and STRM \cite{strm} introduce joint spatio-temporal modeling techniques for robust few-shot matching. Nguyen et al. \cite{nguyen2022inductive} and Huang et al. \cite{huang2022compound} utilize multiple similarity functions to accurately compare videos. MoLo \cite{molo} introduces a motion autodecoder and long-short contrastive objective to explicitly extract motion dynamics. D2ST \cite{d2st} uses an adaptive tuning framework and encode spatial and temporal features in a disentangled manner. \np{HyRSM++} \cite{hyrsm++} \np{HCL} \cite{hcl}

\np{TODO - Add HyRSM to class 2 of models as well (falls in both buckets)? Describe HyRSM++, Describe HCL}
Unlike these previous methods, we blah blah blah...

\subsubsection{Point Tracking} aims to track a set of physical points in a video.
% Given a pixel in a frame, the task of point tracking involves predicting the position and visibility of a world surface point in each frame of a video.
% Sand and Teller \cite{sand2008particle} introduced the concept of ``particle video'', which represents a video with a set of particles that traverse multiple frames, to leverage long-range temporal priors in video motion estimation. This paradigm acts as a bridge between feature tracking \cite{} and optical flow based methods \cite{}. PIPs \cite{harley2022particle} builds on this classic concept to build a model that tracks points through occlusions.
TAP-Vid \cite{doersch2022tap} introduced the problem of tracking any physical point and proposed the TAP benchmark along with a simple baseline method TAPNet. However, this method cannot track occluded points. 
PIPs \cite{harley2022particle} builds on the classic concept of ``particle video'' \cite{sand2008particle} that acts as a bridge between local feature matching \cite{bay2006surf, lowe2004distinctive, detone2018superpoint, shi1994good, tomasi1991detection} and optical flow \cite{neoral2024mft, teed2020raft, dosovitskiy2015flownet, xu2017accurate, zhang2021separable, shi2023videoflow} based methods to leverage long-range temporal priors in video motion estimation. PIPs processes videos in fixed-sized temporal windows and track points through occlusions.
% In addition to persistence through occlusion, PIPs learns multi-frame temporal context 
% The method tracks selected points with a fixed sliding window and restarts from the last frame where the point is visible. However, the model loses the target if it stays occluded beyond the size of the window. 
%  which are challenges in previous methods of trajectory tracking that are based on feature matching and optical flow respectively. 
% Although it learns multi-frame temporal context and can persist through shorter occlusions, PIPs loses the target for longer occlusions that extend beyond the window size.
Although it can persist through shorter occlusions, PIPs loses the target for longer occlusions that extend beyond the window size.
TAPIR \cite{doersch2023tapir} integrates the global matching strategy from TAPNet with the iterative refinement step of PIPs to build a fully-convolutional architecture that achieves enhanced tracking accuracy.
PointOdyssey \cite{zheng2023pointodyssey} addresses long-term tracking with PIPs++, a modification of PIPs that significantly extends its temporal receptive field, and introduces a benchmark for the task of fine-grained long-term tracking.
OmniMotion \cite{wang2023tracking} also addresses per-pixel per-frame trajectory estimation by ensuring global consistency of estimated motion trajectories to produce a method that is robust to occlusions and fast moving objects.
DOT \cite{moing2023dense} proposes a faster and more memory efficient dense point tracking algorithm for use in practice, and combines optical flow with pixel tracking to gain spatial context from correlated pixel trajectories.
While the above methods estimate individual point trajectories independently, CoTracker \cite{cotracker} proposes to jointly estimate point trajectories to take advantage of the correlation between points, resulting in improved performance. It initializes tracks within a window using queried points and refines these trajectories. 
% Inclusion of support points can further improve the performance.
\np{Add more optical flow and feature matching citations - current ones may not be fully relevant} % brox2010large etc from PIPs??

\np{Add to intro?} Previous \textcolor{red}{(not few-shot) action recognition} methods typically rely on optical-flow \cite{piergiovanni2019representation, simonyan2014two, wang2016robust, wang2013action, wang2021weakly, wang2022context, zhu2006action} or frame difference \cite{lee2011vision, wang2021tdn, zhang2012slow} or feature matching \np{I don't see any action recognition papers using feature matching} to learn explicit motion cues for action recognition. Due to the high cost of optical flow, recent approaches investigate extraction of motion features from only raw frame input \cite{dave2022tclr, fan2020rubiksnet, ji20123d, jiang2019stm, kwon2020motionsqueeze, tran2018closer, wang2020video, wang2022long}.

Pairwise optical flow fails to capture motion trajectories over long temporal windows, and sparse feature tracking does not model the motion of all pixels. We adopt the point representation of motion learning/information in our work, which serves as a bridge between optical flow and \textcolor{red}{feature matching}. Specifically, we integrate CoTracker in our method as it can efficiently and jointly track multiple points, ...

% MFT - neoral2024mft
% cotracker

==> tables/molo_speed.tex <==
\begin{table}[t!]

\addtolength{\tabcolsep}{2pt} % Increase the column separation by 5pt
% \begin{tabularx}{\columnwidth}{XXXXXXXXXXXX}
\caption{Comparssion with previous state fo the art in terms on inference speed, GFLOPS, and \emph{trainable} pramaters}
\label{table:speed}
\resizebox{\columnwidth}{!}{

\begin{tabular}{@{}lccc@{}}

\toprule
\textbf{Grid Size} &  \textbf{Inference speed} & \textbf{GFLOPS}  & \textbf{Params}  \\
\midrule

\textbf{MoLo~\cite{molo}} & 0.871s &13.41 &89.6M \\
\textbf{Ours} & 1.051s &23.1 + 16.2 &10.8M \\



\bottomrule
\end{tabular}}

% \end{tabularx}
\end{table}


==> tables/point_and_num_points.tex <==
\begin{table*}[!t]
\begin{minipage}[b]{0.55\linewidth}
\addtolength{\tabcolsep}{2pt} % Increase the column separation by 5pt
% \begin{tabularx}{\columnwidth}{XXXXXXXXXXXX}
\caption{Comparison of uniformly re-initialized point sampling to baseline}
\label{table:four}
\resizebox{12.5cm}{!}{
\begin{tabular}{@{}lccc|ccc@{}}

\toprule
& \multicolumn{3}{c}{\textbf{SSv2-Full}}  & \multicolumn{3}{c}{\textbf{SSv2-Small}}  \\ \cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} 
\textbf{Strategy} & \multicolumn{1}{l}{1-shot} & \multicolumn{1}{l}{3-shot} & \multicolumn{1}{l}{5-shot} & \multicolumn{1}{l}{1-shot} & \multicolumn{1}{l}{3-shot} & \multicolumn{1}{l}{5-shot} \\
\midrule
No points &  56.2 & 68.0 & 72.5 & 44.6 & 57.7 & 62.5 \\ 
First frame only &  56.0 & 68.5 & 73.3 & 46.1 & 57.4 & 63.6 \\ 
Uniform temporal sampling &  \textbf{57.7} & \textbf{70.0 }& \textbf{74.6} & \textbf{47.9} & \textbf{60.0} & \textbf{64.4} \\ 

\bottomrule
\end{tabular}}

\end{minipage}\quad

\begin{minipage}[t]{0.5\linewidth}
\addtolength{\tabcolsep}{2pt} % Increase the column separation by 5pt
% \begin{tabularx}{\columnwidth}{XXXXXXXXXXXX}
\caption{Comparison of different number of sampled points for 1-shot, 3-shot, and 5-shot settings.}
\label{table:five}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
&  \multicolumn{3}{c}{\textbf{SSv2-Full}}  & \multicolumn{3}{c}{\textbf{SSv2-Small}}  \\ \cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} 
\textbf{Points}  & \multicolumn{1}{l}{1-shot} & \multicolumn{1}{l}{3-shot} & \multicolumn{1}{l}{5-shot} & \multicolumn{1}{l}{1-shot} & \multicolumn{1}{l}{3-shot} & \multicolumn{1}{l}{5-shot} \\
\midrule
32 &   53.4 & 66.2 & 71.8 & 44.5 & 57.4 & 61.5\\
64 &   55.5 & 68.3 & 72.5 & 45.7 & 57.7 & 62.0\\
128 &   56.5 & 69.1 & 73.7 & 46.8 & 59.9 & 63.9\\
256 &   \textbf{57.7} & \textbf{70.0} & \textbf{74.6} & \textbf{47.9} & \textbf{60.0} & \text{64.4}\\


\bottomrule
\end{tabular}}
\end{minipage}

\end{table*}




==> tables/trackers.tex <==
\begin{table}[!]
\addtolength{\tabcolsep}{2pt} % Increase the column separation by 5pt
% \begin{tabularx}{\columnwidth}{XXXXXXXXXXXX}
\caption{Comparison of different point trackers for 1-shot, 3-shot, and 5-shot settings.}
\label{table:tracker}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccc|ccc|ccc@{}}
\toprule
&  \multicolumn{3}{c}{\textbf{Kinetics}} & \multicolumn{3}{c}{\textbf{SSv2-Full}}  & \multicolumn{3}{c}{\textbf{SSv2-Small}}  \\ \cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} 
\textbf{Point tracker} &  \multicolumn{1}{l}{1-shot} & \multicolumn{1}{l}{3-shot} & \multicolumn{1}{l}{5-shot} & \multicolumn{1}{l}{1-shot} & \multicolumn{1}{l}{3-shot} & \multicolumn{1}{l}{5-shot} & \multicolumn{1}{l}{1-shot} & \multicolumn{1}{l}{3-shot} & \multicolumn{1}{l}{5-shot} \\
\midrule
TAPIR~\cite{doersch2023tapir} & 80.8 & 88.3 & 90.3 & 56.9 & 69.7 & 73.9 & 47.1 & 58.8 & 64.2\\
PIPS++~\cite{zheng2023pointodyssey} & 82.5 & 89.2 & 90.4 & 57.3 & 70.2 & 74.1 & 47.5 & 59.3 & 64.3\\
CotrackerV2~\cite{cotracker} & 81.9 & 89.9 & 91.1 & 57.7 & 70.0 & 74.6 & 47.9 & 60.0 & 64.4\\

\bottomrule
\end{tabular}}
% \end{tabularx}
\end{table}

